Exascale Grid Optimization (ExaGO) toolkit: An open-source high-performance package for solving large-scale grid optimization problems

This paper introduces the Exascale Grid Optimization (ExaGO) toolkit, a library for solving large-scale alternating current optimal power flow (ACOPF) problems including stochastic effects, security constraints and multi-period constraints. ExaGO can run on parallel distributed memory platforms, including massively parallel hardware accelerators such as graphical processing units (GPUs). We present the details of the ExaGO library including its architecture, formulations, modeling details, and its performance for several optimization applications.

==> figures/intro_fig.tex <==
\tikzstyle{vtx}=[draw,circle,fill,minimum width=1pt]

\tikzstyle{ed}=[color=blue]

\begin{figure}[h!]
    \centering
    \scalebox{.8}{

\begin{tikzpicture}[auto, thick]
   \node (o) at (0,0,0) {};
   \node[label=left:{Security}] (x) at (-6,0,0) {}; 
   \node[label=above:{Stochasticity}] (y) at (0,7,0) {}; 
   \node[label=right:{Time}] (z) at (0,0,-8) {}; 
 % \node[time,label=below:$t_0$] (t0) at (0,0) {};
 % \node[time,label=below:$t_1$] (t1) at (2,0) {};
 % \node[time,label=below:$t_2$] (t2) at (4,0) {};
 % \node[time,label=below:$t_3$] (t3) at (6,0) {};
  
  \node[vtx,label=below:\textbf{OPFLOW}] (opflow) at (0,0,0) {};
  \node[vtx,label=right:\textbf{TCOPFLOW}] (tcopflow) at (0,0,-4) {};
  \node[vtx,label=below:\textbf{SCOPFLOW}] (scopflow) at (-4,0,0) {};
  \node[vtx,label=below:\textbf{SOPFLOW}] (sopflow) at (0,4,0) {};
  

  \node[vtx,label=above:\textbf{SOPFLOW}] (b) at (0,4,-4) {};
  \node[vtx,label=left:\textbf{SOPFLOW}] (c) at (-4,4,0) {};
  \node[vtx,label=above:\textbf{SOPFLOW}] (d) at (-4,4,-4) {};
  
  \path (scopflow) edge [->,thick] (x);
  \path (sopflow) edge [->,thick] (y);
  \path (tcopflow) edge [->,thick] (z);
  
  \path (sopflow) edge [ed] (b);
  \path (sopflow) edge [ed] (c);
  \path (b) edge [ed] (d);
  \path (c) edge [ed] (d);
  
  \path (scopflow) edge [ed] (c);
  \path (tcopflow) edge [ed] (b);
  \path (o) edge [ed] (tcopflow);
  \path (o) edge [ed] (scopflow);
  \path (o) edge [ed] (sopflow);
 % \path (t0) edge (t1);
 % \path (t1) edge (t2);
 % \path (t2) edge (t3);


\end{tikzpicture}}
\caption{\exago provides applications along the dimensions of security (contingencies), time, and stochasticity. The label vertices denote different \exago applications available.}
\label{fig:intro_fig}
    
\end{figure}

==> sctopflow_fig.tex <==
\definecolor{lavander}{cmyk}{0,0.48,0,0}
\definecolor{violet}{cmyk}{0.79,0.88,0,0}
\definecolor{burntorange}{cmyk}{0,0.52,1,0}

\def\lav{lavander!90}
\def\oran{orange!30}

\tikzstyle{time}=[draw,circle,violet,bottom color=\lav,
                  top color= white, text=violet,minimum width=20pt]
                  
\tikzstyle{base}=[draw,circle,burntorange, left color=\oran,
                       text=violet,minimum width=20pt]

\begin{figure}[h!]
\centering
\begin{tikzpicture}[auto, thick]
  % scenario 0
  \node[base,label=below:$t_0$] (s0c0t0) at (0,2) {};
  \node[time,label=below:$t_1$] (s0c0t1) at (2,2) {};
  \node[time,label=below:$t_2$] (s0c0t2) at (4,2) {};
  \node[time,label=below:$t_3$] (s0c0t3) at (6,2) {};
  
  \path (s0c0t0) edge (s0c0t1);
  \path (s0c0t1) edge (s0c0t2);
  \path (s0c0t2) edge (s0c0t3);
  
  % contingency rectangle from (-0.5,1.5) to (6.5,2.5)
   \node[draw,rectangle,dashed,minimum width=7cm,minimum height=1cm,label=left:{$\mathbf{c_0}$}] (s0) at (3.0,2.0) {};
  
  \node[time,label=below:$t_0$] (s0c1t0) at (0,0) {};
  \node[time,label=below:$t_1$] (s0c1t1) at (2,0) {};
  \node[time,label=below:$t_2$] (s0c1t2) at (4,0) {};
  \node[time,label=below:$t_3$] (s0c1t3) at (6,0) {};
  
  \path (s0c1t0) edge (s0c1t1);
  \path (s0c1t1) edge (s0c1t2);
  \path (s0c1t2) edge (s0c1t3);
  
  % contingency rectangle from (-0.5,-0.5) to (6.5,0.5)
   \node[draw,rectangle,dashed,minimum width=7cm,minimum height=1cm,label=left:{$\mathbf{c_1}$}] (s0) at (3.0,0.0) {};
  
   \path (s0c0t0) edge [bend right,color=red] (s0c1t0);
  
  % scenario rectangle from (-1.0,-0.75) to (7.0,2.75)
   \node[draw,rectangle,dotted,minimum width=8cm,minimum height=3.5cm,label=left:{$\mathbf{s_0}$}] (s0) at (3.0,1.0) {}; 
  
  % scenario 1
  \node[base,label=below:$t_0$] (s1c0t0) at (0,4) {};
  \node[time,label=below:$t_1$] (s1c0t1) at (2,4) {};
  \node[time,label=below:$t_2$] (s1c0t2) at (4,4) {};
  \node[time,label=below:$t_3$] (s1c0t3) at (6,4) {};
  
  \path (s1c0t0) edge (s1c0t1);
  \path (s1c0t1) edge (s1c0t2);
  \path (s1c0t2) edge (s1c0t3);
  
   % contingency rectangle from (-0.5,3.5) to (6.5,4.5)
   \node[draw,rectangle,dashed,minimum width=7cm,minimum height=1cm,label=left:{$\mathbf{c_0}$}] (s0) at (3.0,4.0) {};
  
  \node[time,label=below:$t_0$] (s1c1t0) at (0,6) {};
  \node[time,label=below:$t_1$] (s1c1t1) at (2,6) {};
  \node[time,label=below:$t_2$] (s1c1t2) at (4,6) {};
  \node[time,label=below:$t_3$] (s1c1t3) at (6,6) {};
  
  \path (s1c1t0) edge (s1c1t1);
  \path (s1c1t1) edge (s1c1t2);
  \path (s1c1t2) edge (s1c1t3);
  
   % contingency rectangle from (-0.5,5.5) to (6.5,6.5)
   \node[draw,rectangle,dashed,minimum width=7cm,minimum height=1cm,label=left:{$\mathbf{c_1}$}] (s0) at (3.0,6.0) {};
  
  \path (s1c0t0) edge [bend left,color=red] (s1c1t0);
  
  \path (s0c0t0) edge [bend left,ultra thick,color=blue] (s1c0t0);
  
   % scenario rectangle from (-1.0,3.75) to (7.0,6.75)
   \node[draw,rectangle,dotted,minimum width=8cm,minimum height=3.5cm,label=left:{$\mathbf{s_1}$}] (s1) at (3.0,5.0) {};
  

\end{tikzpicture}
\caption{Stochastic multi-period contingency constrained example with two scenarios $s_0$ and $s_1$. Each scenario has two contingencies $c_0$,$c_1$ and each contingency consists of four time-periods $t_0$, $t_1$, $t_2$, $t_3$. State $s_0,c_0,t_0$ represent the base case (no contingency) case for the two scenarios.  We assume that any contingency is incident at the first time-step, i.e., at $t_0$. Thus, the contingency states $c_1,t_0$ is coupled with the no-contingency state $c_0,t_0$ at time $t_0$ for both the scenarios. The {\textcolor{red}{red}} line denotes the coupling between the contingency and the no-contingency states.The {\textcolor{blue}{blue}} line denotes the coupling between the scenarios}
\label{fig:sctopflow}
\end{figure}

==> topflow_fig.tex <==
\definecolor{lavander}{cmyk}{0,0.48,0,0}
\definecolor{violet}{cmyk}{0.79,0.88,0,0}
\definecolor{burntorange}{cmyk}{0,0.52,1,0}

\def\lav{lavander!90}
\def\oran{orange!30}

\tikzstyle{time}=[draw,circle,violet,bottom color=\lav,
                  top color= white, text=violet,minimum width=20pt]
\tikzstyle{base}=[draw,circle,burntorange, left color=\oran,
                       text=violet,minimum width=20pt]

\begin{figure}[h!]
\centering
\begin{tikzpicture}[auto, thick]
  \node[time,label=below:$t_0$] (t0) at (0,0) {};
  \node[time,label=below:$t_1$] (t1) at (2,0) {};
  \node[time,label=below:$t_2$] (t2) at (4,0) {};
  \node[time,label=below:$t_3$] (t3) at (6,0) {};
  
  \path (t0) edge (t1);
  \path (t1) edge (t2);
  \path (t2) edge (t3);


\end{tikzpicture}
\caption{Multi-period optimal power flow example with four time-steps. The lines connecting the different time-periods denote the coupling between them.}
\label{fig:tcopflow}
\end{figure}
